Conning the Crypto Conman: End-to-End Analysis of Cryptocurrency-based Technical Support Scams

The mainstream adoption of cryptocurrencies has led to a surge in wallet-related issues reported by ordinary users on social media platforms. In parallel, there is an increase in an emerging fraud trend called cryptocurrency-based technical support scam, in which fraudsters offer fake wallet recovery services and target users experiencing wallet-related issues. In this paper, we perform a comprehensive study of cryptocurrency-based technical support scams. We present an analysis apparatus called HoneyTweet to analyze this kind of scam. Through HoneyTweet, we lure over 9K scammers by posting 25K fake wallet support tweets (so-called honey tweets). We then deploy automated systems to interact with scammers to analyze their modus operandi. In our experiments, we observe that scammers use Twitter as a starting point for the scam, after which they pivot to other communication channels (eg email, Instagram, or Telegram) to complete the fraud activity. We track scammers across those communication channels and bait them into revealing their payment methods. Based on the modes of payment, we uncover two categories of scammers that either request secret key phrase submissions from their victims or direct payments to their digital wallets. Furthermore, we obtain scam confirmation by deploying honey wallet addresses and validating private key theft. We also collaborate with the prominent payment service provider by sharing scammer data collections. The payment service provider feedback was consistent with our findings, thereby supporting our methodology and results. By consolidating our analysis across various vantage points, we provide an end-to-end scam lifecycle analysis and propose recommendations for scam mitigation.

==> evaluate_scammer_profile_information.tex <==
\subsection{Scammer User Detail }
\label{sec:evaluate_scam_mechanics}
In this section, We further dive deep into the user detail of scammers.

\textbf{Following Count} Our dataset show that scammers prefer \emph{Following} targeted victims. By \emph{Following}, allows the scammer to track public information such as \emph{likes} and \emph{comments} performed by the victim. The median \emph{Following} count for scammers from Twitter and Instagram was found to be 11 and 25 respectively. We arrange the scammer based on the chronological order of first seen in our database in Fig ~\ref{fig:insta_twitter_following_posts}. (a) and (b) and display \emph{Following} count for Twitter and Instagram accounts.

\textbf{Posts Count}
Fig \ref{fig:insta_twitter_following_posts} (a) and (c) shows that scammer prefers to interact via \emph{Posts} on Twitter whereas \emph{Following} users via Instagram. The median \emph{posts} count for Instagram was found to be 5  whereas for Twitter the collated median count for \emph{replies}, \emph{retweets}, and \emph{quoted} tweets showed to 7.


 \begin{figure*}[ht!]
            \includegraphics[width=.33\textwidth]{images/fig6a.pdf}\hfill
            \includegraphics[width=.33\textwidth]{images/fig6b.pdf}\hfill           \includegraphics[width=.33\textwidth]{images/fig6c.pdf}
            \caption{\emph{Instagram and Twitter scammer accounts breakdown by Following and Posts interaction count chronologically.}} 
         \label{fig:insta_twitter_following_posts}
\end{figure*}


==> evaluate_targeted_wallets.tex <==
\begin{figure}[htp]
\centering
\includegraphics[width=.48\textwidth]{images/wallet_target_forms.png}\hfill
\caption{ \emph{Scamming Google forms targeting wallet users - These are examples of Google forms where scammers ask the user to release private key phrases as part of fake support. The left image is targeted to customer of MetaMask wallet, middle to Coinbase wallet and right to Trust wallet customer.}}
\label{fig:wallet_target_forms}
\end{figure}


\subsection{Targeted Wallet via Fake Support Media}\label{sec:pivoting}
Our study shows that scammer asks users to contact them via unofficial channels for fake support. These support communication channels are in the form of Email, Twitter, Instagram, Telegram, WhatsApp, and Google Forms URLs. We refer to these unofficial channels of communication as scam media. An example of tweet interaction via quoted tweets where a scammer asks the user to further contact via an external communication medium is shown in Fig. ~\ref{fig:scam_media}. 

\emph{Replies} and \emph{Quoted Tweets} are the two forms of interaction mechanics that allow sharing of short messages on Twitter. By analyzing these messages from scammers in the form of replies and quoted tweets, we identified the distribution of scam media. In table ~\ref{table:wallet_target_breakdown} we provide the breakdown of distinct scam media targeting the wallet type based on tweet posts by \emph{HoneyTweet} module. In total, out of 28428 replies and 10218 quoted tweets messages, 3098 distinct scam media were distributed by 9149 scammers targeting 10 ten different wallets. Among 10 wallets, highlighted in bolded red color, Trust Wallet (29.89\%), Coinbase (27.50\%), and MetaMask (26.62\%) were found to be the top three targets of scammers whereas Badger (8.45\%) and Free Wallet (8.05\%) were the lowest in scam target by the overall category. We find some wallets are specifically targeted more than others by the types of scam media. We highlight the most preferred scam media targeting the wallet type in bolded blue color in table ~\ref{table:wallet_target_breakdown}. It shows scammers ask users of Binance to chat via Instagram and Telegram direct messaging whereas users of Coinbase and MetaMask wallet are asked to contact via Google Forms URLs. An example of a Google Forms URL where users are asked to release private key phrases of a wallet is shown in figure ~\ref{fig:wallet_target_forms}. Overall, the scammer's preference of using scam media type for fake support showed that 34.73\% are targeted via Google Forms URLs, and the rest other by direct messaging features through Instagram, Telegram, Twitter, WhatsApp, and Email.    





==> evaluate_tweet_interaction.tex <==
\subsection{Scam Mechanics}
\label{sec:evaluate_tweet_interaction}

\textbf{Overview }
The table \ref{table:over_all_tweet_interact} shows the breakdown of tweets interacted by scammers upon posted by \emph{HoneyTweet} module. The first column shows various ways users interact with the tweet posts ~\cite{definitiontweet}. We call column one as \emph{scam mechanics} performed by scammers to gain the attention of the victim. The second column shows the total count found in each scam mechanic. The third column is the distinct count of each scam mechanic. Twitter provides a unique identifier upon the creation of posts, for each of the scam mechanics the unique identifier \emph{TweetID} associated is shown by column four. Upon such interaction, we saw the scammers are suspended by Twitter upon any violation of Twitter's policy or report due to abuse history. Such \emph{suspended} scamming accounts are displayed in column 5. Similarly, those accounts which were inactive due to deactivation or deletion by the scammer themselves are shown in column 6. The total number of scammer accounts found is shown in the last column seven. Overall, 9149 scamming accounts interacted with 20740 unique honey tweets from the total of 25000 unique honey tweets posted by \emph{HoneyTweet} module. Thus, 79.42\% of honey tweets posted resulted in one or more forms of interaction from scammers. 

Fig. ~\ref{fig:scammer_interaction_with_honey_tweet} shows overall interaction by scammers with our \emph{HoneyTweet} module. The first graph Fig. ~\ref{fig:scammer_interaction_with_honey_tweet}(a) shows the continuous growth of scammers interacting with our system over the experiment time. The cdf representation of the breakdown of scammer account interaction with our honey tweets in the forms of \emph{Replies}, \emph{Quoted Tweets}, \emph{Retweets}, and \emph{Likes} is depicted by the second graph Fig. ~\ref{fig:scammer_interaction_with_honey_tweet}(b). During our experiment, we found that scamming accounts follow our four honey accounts which are shown in Fig. ~\ref{fig:scammer_interaction_with_honey_tweet}(c). We further explain each scam mechanics in the below bulleted points.  
\begin{itemize}
\item \textbf{Replies} allows users to respond to the posted tweets. Our results show that  86.92\% of scammers who interacted with \emph{HoneyTweet} preferred to interact by replying to the potential victim's tweet. Prior to getting suspended by Twitter because of an abuse report or violation of Twitter's policy, 64.23\% of replying scamming accounts were found to perform 28424 responses to 45.61\% of interacted honey tweets.     

\item \textbf{Retweets} allows users to re-post an already tweeted post. Our results show that retweets are among the least preferred scam mechanics. 0.5\% of scammers retweeted 6.4\% of distinct honey tweets. It is to be noted that retweet does not offer direct interaction to the potential victim but rather allows the scammer's timeline to share publicly to followers of the scammer who might be potentially targeting these retweets as the source for scamming. This also provides a gesture to the potential victim that someone actually cared to share their tweets publicly.  

 \begin{figure*}[ht!]
    \includegraphics[width=1.0\textwidth]{images/scam_media.png}\hfill
            \caption{\emph{Scammer asking potential victims to reach via unofficial channels (Email, Instagram, and Google Forms) of communication for fake support - This graph shows how scammers pivot the users to contact via other social media as part of fake support.}} 
         \label{fig:scam_media}
\end{figure*}

\item \textbf{Quoted Tweets} provide users to share someone else tweets by adding a comment. Out of 20740 interacted honey tweets, 26.60\% scamming accounts shared 25.08\% of honey tweets. We observed Twitter's ability to suspend quoting scamming users to 62.32\%, the lowest of all scam mechanics suspending accounts category. 

\item \textbf{Likes} is the heart icon that shows someone appreciates the tweet. 41.61\% of suspended scamming accounts perform \emph{Likes} to 48.06\% interacted tweets. We found the scammers perform a combination of \emph{Likes} with \emph{Replies} or \emph{Quoted Tweets}.  

\item \textbf{Follows} provides subscribing tweets from the preferred users. Out of 660 scamming accounts followed by four honey tweet accounts, 398 were found to be suspended by Twitter. The following accounts not only followed four different honey accounts but also interacted with 48.06\% of distinct honey tweets. Following potential victim not only allows scammers to keep track of the user's timeline but also potentially encourage the user to follow the scammer back which is another way for a scammer in thwarting Twitter's blocking against the suspicious or never-before-interacted account.
\end{itemize}

 \begin{figure*}[ht!]
            \includegraphics[width=.33\textwidth]{images/all_active_tweets_scam_account_interaction.png}\hfill           \includegraphics[width=.33\textwidth]{images/honey_account_follower_daily_followers.png}
            \includegraphics[width=.33\textwidth]{images/daily_new_scammer_data.png}\hfill
            \caption{\emph{Scammer Interaction with HoneyTweet Module - In this graph we display the scammer's interaction with \emph{HoneyTweet module}. The left graph shows the overall interaction in the form of replies, retweets, quoted tweets, and likes seen over the span of the experiment time. The middle graph shows the scammer \emph{following} the four honey Twitter accounts. The right graph shows the cumulative sum of scammers based on interaction with our posts.}} 
         \label{fig:scammer_interaction_with_honey_tweet}
\end{figure*}




==> evaluate_user_detail_and_timelines.tex <==
The scammer user account interacted with \emph{HoneyTweet} is fed into \emph{Timelines module} in order to collect the account's aliveness and monitor their interaction in the wild. In this section, we dive deep into providing analysis of scammer user detail, and association in tweet interaction via observing the timelines of scammer. 

\input{evaluate_user_detail}
\input{profile_picture_analysis}
\input{evaluation_of_scammers_timeline}


==> evaluating_scammers_profile_image.tex <==
\subsection{Analysis of Profile Picture of Scammers}
\label{sec:evaluate_profile_pic}

==> images/mainflow.tex <==
% \section{Diagrammatic view of Multisketch operations}\label{app:mainflow}  

% A user registers with a user id $\u$ and a vector of biometric templates
% $\mvec=\mvecss{\mlen}$. Multisketch uses two databases $\dbid$ and $\dbmsg$\@,
% where $\dbid$ contains user id $\u$ and the corresponding helper data
% $\sketchval$, and $\dbmsg$ contains the random permutation of the templates
% registered so far. Highlighted are the entries corresponding to a user $\u_4$
% with templates $\mvec_4=\mvec_{41}\ldots\mvec_{4\mlen}$.% and helper
%     % data $\sketchval_4$.
\begin{figure}[t]
  \centering
  \begin{tikzpicture}[
    >=stealth,
    node distance=2cm,
    database/.style={
      cylinder,
      cylinder uses custom fill,
      cylinder body fill=black!25!white,
      cylinder end fill=black!25!white,
      shape border rotate=90,
      aspect=0.25,
      minimum width=2em,
      minimum height=2em,
      draw
    },
    func/.style={
      rectangle,
      fill=red!25!white,
      minimum width=1cm,
      minimum height=1em,
      draw
    },
    cell/.style={
      rectangle,
      draw=black!50!white
    }
    ]
    \node (user) at (0, 0) {User};
    \node[func, right of=user, right=-1.1em, above=3em] (msketch) {$\MS$}; 
    \draw[below of=msketch, dashed, anchor=west] (.85,0.55) rectangle (5.9,-1.2); 
    \node[func, below of=msketch, anchor=east, below=1.95cm,fill=red!10!white,dashed] (mrecover) {$\MRec$};
    % \node[database, right of=user, anchor=south, above=1em, right=2cm] (db1) {$\dbid$};
    \matrix (db1) [right of=user, anchor=south, below=2pt, right=-0.1cm, 
    matrix of math nodes,
    column sep = -\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}}, 
    column 2/.style={nodes={cell}}, 
    anchor=west] {
      \u_1 & \sketchval_1\\
      \u_2 & \sketchval_2\\
      \u_3 & \sketchval_3\\
      |[draw,fill=blue!20]|\u_4 & |[draw,fill=blue!20]|\sketchval_4\\
    };
    \node[left of=db1, anchor=east,right=1.1cm] {$\dbid$};
    \matrix (db2) [right of=db1, left=25pt, matrix of math nodes,
    column sep = 2\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}},
    column 2/.style={nodes={cell}}, 
    column 3/.style={nodes={cell}}, 
    column 4/.style={nodes={cell}}, 
    column 5/.style={nodes={cell}}, 
    anchor=west] {
      \mvec_{21} &\mvec_{12} & |[draw,fill=blue!20]|\mvec_{43} &  & \mvec_{3\mlen} \\
      |[draw,fill=blue!20]|\mvec_{41} &\mvec_{32} & \mvec_{33} & |[draw=white]|\ldots & \mvec_{2\mlen} \\
      \mvec_{11} &|[draw,fill=blue!20]|\mvec_{42} & \mvec_{23} &  & \mvec_{1\mlen} \\
      \mvec_{31} &\mvec_{22} & \mvec_{13} & & |[draw,fill=blue!20]|\mvec_{4\mlen} \\
    };
    \node[left of=db2, left=-4pt] {$\dbmsg$};

    % \node[database,right of=db1] (db2) {$\dbmsg$};
    \node[func,below of=db1,anchor=north,above=8pt,left=8pt] (gu) {GetUser};
    \node[func,right of=gu,anchor=east,right=-5pt] (fm) {FindMatches};
    \node[func,below of=db1,anchor=east,below=2em,right=-3pt] (recover) {Recover};

    \draw[->,blue!50,thick] (user.north) |- node[black,near end,above]{$u, \mvec$} node[black,near end,below,font=\small]{register} 
    (msketch.west);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$u, \sketchval$} (db1);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$\mvec$} (db2);

    \draw[->,blue!50,thick] (user.south) |- ++(1,-0.9) node[black,near end,above]{$u, \mvectilde$} node[black,near end,below,font=\small]{login}   -| node[black,left,near end]{$u$}
    (gu.north);
    \draw[->,blue!50,thick] (user.south) |- ++(0,-0.9)  -- ++(3.1,0) |- node[black,near end, above]{$\mvectilde$}
    (fm.west);
    \draw[->,blue!50,thick] (db1.south) |- node[black,near end,above]{} (gu.east);
    \draw[->,blue!50,thick] (db2.south) |- node[black,near end,above]{} (fm.east);
    \draw[->,blue!50,thick] (gu.south) |- node[black,near end,above]{$\sketchval$} (recover.west);
    \draw[->,blue!50,thick] (fm.south) |- node[black,near end,above]{$\mvec'$} (recover.east);    
    \draw[->,blue!50,line width=2pt] (recover.south) -- node[black,near end,right]{$\mvec$ or $\bot$} ++(0, -0.65);
  \end{tikzpicture}
  % \rcnote{Rough sketch of the flow of the \biosketch.} 
  \caption{Diagram of multisketch as a part of an authentication service. 
  }
  \label{fig:mainflow}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

